Toward the van Benthem Characterization Theorem for Non-Distributive Modal Logic

In this paper, we introduce the simulations and bisimulations on polarity-based semantics for non-distributive modal logic, which are natural generalizations of those notions on Kripke semantics for modal logic. We also generalize other important model-theoretic notions about Kripke semantics such as image-finite models, modally-saturated models, ultrafilter extension and ultrapower extension to the non-distributive setting. By using these generalizations, we prove the Hennessy-Milner theorem and the van Benthem characterization theorem for non-distributive modal logic based on polarity-based semantics.

==> wastepaper.tex <==
{{\centering
\begin{tabular}{ccccccccccccc}
     $p \vdash p$ & \quad\quad & $\bot \vdash p$ & \quad\quad & $p \vdash p \vee q$ & \quad\quad & $p \wedge q \vdash p$ & \quad\quad & $\top \vdash \Box\top$ & \quad\quad & $\Box p \wedge \Box q \vdash \Box(p \wedge q)$
     \\
     & \quad & $p \vdash \top$ & \quad & $q \vdash p \vee q$ & \quad & $p \wedge q \vdash q$ &\quad &  $\Diamond\bot \vdash \bot$ & \quad & $\Diamond(p \vee q) \vdash \Diamond p \vee \Diamond q$\\
     & \quad & & \quad &  & \quad &  &\quad &  
\end{tabular}
\par}}

{{\centering
\small
\begin{tabular}{llcll}
$\mathfrak{M}, a \Vdash \Box\phi$ &  iff $(\forall x\in X)(\mathfrak{M}, x \succ \phi \Rightarrow a R_\Box x)$ & \quad\quad &
$\mathfrak{M}, x \succ \Box\phi$ &  iff $(\forall a\in A)(\mathfrak{M}, a \Vdash \Box\phi \Rightarrow a I x)$\\
%
$\mathfrak{M}, x \succ \Diamond\phi$ &  iff for all $ a\in A$, if $\mathfrak{M}, a \Vdash \phi$ then $x R_\Diamond a$ &&
$\mathfrak{M}, a \Vdash \Diamond\phi$ & iff $(\forall x\in X)(\mathfrak{M}, x \succ \Diamond\phi \Rightarrow a I x)$.  \\
\end{tabular}
\par}}
\smallskip


\[
\mathfrak{M}, a \Vdash p\ \mathrm{iff}\ a\in \val{p}_{\mathfrak{M}}.
\quad
\mathfrak{M}, x \succ p\ \mathrm{iff}\ x\in \descr{p}_{\mathfrak{M}}.
\quad
\mathfrak{M}, a \Vdash\top\ \mathrm{always}.
\quad
\mathfrak{M}, x \succ  \bot\ \mathrm{always}.
\]
\[
\mathfrak{M}, x \succ \top\ \mathrm{iff}\ (\forall x\in A)aIx. \quad
\mathfrak{M}, a\Vdash\bot\ \mathrm{iff}\ (\forall x\in X)aIx.
\]
\[
\mathfrak{M}, a \Vdash \varphi\wedge \psi \ \mathrm{iff}\ \mathfrak{M}, a\Vdash \varphi \ \mathrm{and}\ \mathfrak{M}, a \Vdash  \psi\quad
\mathfrak{M}, x \succ \varphi\wedge \psi \mathrm{iff}\ (\forall a\in A)(\mathfrak{M}, a \Vdash \varphi\wedge \psi \Rightarrow a I x).
\]

\[
\mathfrak{M}, a \Vdash \Box\varphi\  \mathrm{iff}\  (\forall x\in X)(\mathfrak{M}, x \succ \varphi \Rightarrow a R_\Box x).\quad\mathfrak{M}, x \succ \Box\varphi \ \mathrm{iff}\ (\forall a\in A)(\mathfrak{M}, a \Vdash \Box\varphi \Rightarrow a I x).
\]
\[
\mathfrak{M}, x \succ \Diamond\varphi\ \mathrm{iff}\ (\forall a\in A)(\mathfrak{M}, a \Vdash \varphi \Rightarrow x R_\Diamond a).\quad
\mathfrak{M}, a \Vdash \Diamond\varphi\ \mathrm{iff}\ (\forall x\in X)(\mathfrak{M}, x \succ \Diamond\varphi \Rightarrow a I x).
\]



\begin{definition}
  A two sorted first-order formula $\varphi(g)$ (resp.~$\varphi(m)$) in $\mathcal{L}^1$ is {\em bisimilarity invariant} if and only if for all $\mathrm{LE}$-models $\mathfrak{M}_1$ and $\mathfrak{M}_2$ and all $a_1$ in $\mathfrak{M}_1$, $a_2$ in $\mathfrak{M}_2$ (resp.~$x_1$ in $\mathfrak{M}_1$, $x_2$ in $\mathfrak{M}_2$), and $a_1$, $a_2$ are bisimilar (resp.~$x_1$, $x_2$ are bisimilar), we have $\mathfrak{M}_1\vDash\varphi[a_1]$ if and only if $\mathfrak{M}_2\vDash\varphi[a_2]$ (resp.~$\mathfrak{M}_1\vDash\varphi[x_1]$ if and only if $\mathfrak{M}_2\vDash\varphi[x_2]$).
\end{definition}
